Watermarking Graph Neural Networks based on Backdoor Attacks

Graph Neural Networks (GNNs) have achieved promising performance in various real-world applications. Building a powerful GNN model is not a trivial task, as it requires a large amount of training data, powerful computing resources, and human expertise in fine-tuning the model. Moreover, with the development of adversarial attacks, e.g., model stealing attacks, GNNs raise challenges to model authentication. To avoid copyright infringement on GNNs, verifying the ownership of the GNN models is necessary. This paper presents a watermarking framework for GNNs for both graph and node classification tasks. We 1) design two strategies to generate watermarked data for the graph classification task and one for the node classification task, 2) embed the watermark into the host model through training to obtain the watermarked GNN model, and 3) verify the ownership of the suspicious model in a black-box setting. The experiments show that our framework can verify the ownership of GNN models with a very high probability (up to $99\%$) for both tasks. Finally, we experimentally show that our watermarking approach is robust against a state-of-the-art model extraction technique and four state-of-the-art defenses against backdoor attacks.

==> sections/5_related_work.tex <==
\section{Related Work}
\label{sec:related}

\textbf{Watermarking neural networks.} In addition to being used to hide the secret information into the multimedia signal to protect the copyright of those multimedia data, digital watermarking is also applied to protect the ownership of the neural networks. Recently, there have been several works that studied watermarking for deep neural networks.%~\cite{DBLP:conf/mir/UchidaNSS17, DBLP:conf/uss/AdiBCPK18, DBLP:conf/ccs/ZhangGJWSHM18, DBLP:conf/aaai/ZhangCLFZZCY20}. 
Uchida et al. used a parameter regularizer to embed a watermark in model parameters~\cite{uchida2017embedding}. One limitation of this work is that it assumes the suspicious models can be accessible to extract all the parameters, which is not practical because the stolen models are usually used in a black-box setting, and it will be hard to get access to the models' architecture and parameters directly. Adi et al. used random training instances and random labels to watermark a neural network in a black-box way~\cite{adi2018turning}. This work is more related to ours since they also designed a backdoor attack to implement a watermarking neural network model. However, this work focuses on deep neural networks, which is different from the scenario we consider: verifying the ownership of graph neural networks. Zhang et al. investigated three DNN-applicable watermark generation algorithms~\cite{zhang2018protecting}. Their work proposed a watermark implanting approach to infuse the watermark into deep learning models, and they remotely verified the ownership of DNN models.
Zhang et al. leveraged the spatial invisible watermarking mechanism to protect image processing models~\cite{zhang2020model}. To enable watermarks from binary bits to high-resolution images, both traditional and deep spatial invisible watermarking mechanisms were used.
%proposed a deep invisible watermarking technique to enable high-capacity watermarks for image processing networks.

All the methods mentioned above focus on the watermarking techniques for deep neural networks. Recently, there has been one work investigating watermarking graph neural networks~\cite{zhao2021watermarking}, but this research direction is still under-studied. Zhao et al.~\cite{zhao2021watermarking} presented a watermarking framework for GNNs by generating a random graph associated with features and labels as the trigger input. However, the work focuses on watermarking graph neural networks on the node classification task, while in our paper, we also design watermarking framework for GNNs on the graph classification task.

\textbf{Backdoor attacks in GNNs.} A number of papers have conducted backdoor attacks on GNNs. Zhang et al. proposed a subgraph-based backdoor attack to GNNs for the graph classification task~\cite{zhang2021backdoor}. Xi et al. presented a subgraph-based backdoor attack to GNNs, but this attack can be instantiated for both node classification and graph classification tasks~\cite{xi2021graph}. Xu et al.~\cite{xu2021explainability} conducted research on the explainability of the impact of trigger injecting position on the performance of backdoor attacks on GNNs, and they also proposed a new backdoor attack strategy for the node classification task. %While backdoor attacks in GNNs are undesirable in most settings, we see here that they can be turned into a defense mechanism by applying it to the task of watermarking GNN models.


==> sections/remove_part.tex <==
\iffalse
\textbf{Robustness on the model difference.} As discussed in Section~\ref{threat_model}, we have no access and knowledge about the suspicious model $m^{'}$. Therefore, the suspicious model is likely to have a different architecture from the host model $m$, i.e., $m$ and $m^{'}$ are two different GNN models. An ideal watermarking framework should still be effective when the suspicious model is different from the host model, i.e., the watermarking framework should be robust to the model architecture difference.
Figures~\ref{fig:fig8} and~\ref{fig:fig9} show the accuracy difference of the host model $m$ and different suspicious model $m^{'}$ on the watermarked data, for the NCI1 and COLLAB datasets, respectively. Here, $T$ represents the host model trained with the watermarked data generated by embedding the watermark into sampled training data, while $R$ represents the host model trained with the watermarked data generated by embedding the watermark into generated random graphs. It is obvious from Figures~\ref{fig:fig8} and~\ref{fig:fig9} that for both datasets, the watermarking mechanism based on the second watermarked data generation strategy still has promising performance, i.e., nearly $100\%$ on the accuracy difference, which is significantly higher than that of the first strategy. Especially when the host model is GIN, the accuracy difference of the second strategy and the COLLAB dataset is twice as large as that of the first strategy. This again emphasizes the superior performance of watermarking mechanism based on embedding watermarks into random graphs.

Table~\ref{Table:6} shows the accuracy difference of different host and suspicious models on the watermarked data for the node classification task. 
As we can see, the accuracy difference is still high (more than $90\%$) even if the suspicious model is different from the host model. Therefore, our watermarking framework is robust to the architecture difference between the host and suspicious models.

\begin{figure*}[!ht]
\begin{subfigure}{0.29\textwidth}
  \centering
  \includegraphics[width=\textwidth, page=15]{figs_final_croped.pdf}  
  \caption{}
  \label{fig:fig8-a}
\end{subfigure}
\hfill
\begin{subfigure}{0.29\textwidth}
  \centering
  % include second image
  \includegraphics[width=\textwidth, page=16]{figs_final_croped.pdf}  
  \caption{}
  \label{fig:fig8-b}
\end{subfigure}
\hfill
\begin{subfigure}{0.36\textwidth}
  \centering
  % include second image
  \includegraphics[width=\textwidth, page=17]{figs_final_croped.pdf}  
  \caption{}
  \label{fig:fig8-c}
\end{subfigure}
\caption{Accuracy difference of different suspicious models on two kinds of watermarked data for NCI1 dataset, with host model of DiffPool (a), GIN( b), GraphSAGE (c).}
\label{fig:fig8}
\end{figure*}

\begin{figure*}[!ht]
\begin{subfigure}{0.29\textwidth}
  \centering
  \includegraphics[width=\textwidth, page=18]{figs_final_croped.pdf}  
  \caption{}
  \label{fig:fig9-a}
\end{subfigure}
\hfill
\begin{subfigure}{0.29\textwidth}
  \centering
  % include second image
  \includegraphics[width=\textwidth, page=19]{figs_final_croped.pdf}  
  \caption{}
  \label{fig:fig9-b}
\end{subfigure}
\hfill
\begin{subfigure}{0.36\textwidth}
  \centering
  % include second image
  \includegraphics[width=\textwidth, page=20]{figs_final_croped.pdf}  
  \caption{}
  \label{fig:fig9-c}
\end{subfigure}
\caption{Accuracy difference of different suspicious models on two kinds of watermarked data for COLLAB dataset, with host model of DiffPool (a), GIN (b), GraphSAGE (c).}
\label{fig:fig9}
\end{figure*}

\begin{table}[!ht]
\small
 \centering
 \caption{Accuracy difference of different suspicious models on watermarked data for node classification task}
\begin{tabular}{M{40pt}|M{30pt}|M{50pt}|M{50pt}}
 \hline
\multicolumn{2}{c|}{Accuracy Difference(\%)} & \multicolumn{2}{c}{Suspicious model} \\
\cline{3-4}
\multicolumn{2}{c|}{$Cora | CiteSeer$} & {GCN} & {GAT} \\
\hline
\multirow{2}{*}{Host model} & {GCN} & $97.90 \;\ 99.78$ & $97.76 \;\ 100.0$ \\
 \cline{2-4}
 & {GAT} & $90.17 \;\ 98.79$ & $90.42 \;\ 99.25$ \\
 \hline
\end{tabular}
\label{Table:6}
\end{table}
\fi


\iffalse
\begin{table} [!ht]
\small
 \centering
 \caption{Accuracy difference on watermarked data after fine-tuning for the node classification task}
\begin{tabular}{M{75pt}|M{40pt}|M{40pt}}
 \hline
{Accuracy Difference} & {GCN} & {GAT} \\
 \hline
 \hline
 $Cora$ & $95.28\%$ & $89.93\%$  \\
 \hline
 $CiteSeer$ & $99.62\%$ & $99.04\%$ \\
 \hline
\end{tabular}
\label{Table:9}
\end{table}

\begin{table}
\small
 \centering
 \caption{Test accuracy after fine-tuning for the node classification task}
\begin{tabular}{M{75pt}|M{40pt}|M{40pt}}
 \hline
{Test Accuracy} & {GCN} & {GAT} \\
 \hline
 \hline
 $Cora$ & $82.95\%$ & $86.73\%$  \\
 \hline
 $CiteSeer$ & $77.07\%$ & $79.96\%$ \\
 \hline
\end{tabular}
\label{Table:10}
\end{table}
\fi

\begin{table*}[!ht]
\small
 \centering
 \caption{Test accuracy and attack success rate difference after model pruning for graph classification task (COLLAB, W\_t)}
\begin{tabular}{c|c|c|c|c|c|c}
 \hline
\multirow{2}{*}{Pruning rate} & \multicolumn{2}{c|}{DiffPool} & \multicolumn{2}{c|}{GIN} & \multicolumn{2}{c}{GraphSAGE} \\
\cline{2-7}
 & {Test Acc.} & {Watermark Acc. Diff.} & {Test Acc.} & {Watermark Acc. Diff.} & {Test Acc.} & {Watermark Acc. Diff.}\\
\hline
{$0\%$} & {$80.36\%$} & {$74.16\%$} & {$81.46\%$} & {$70.47\%$} & {$79.59\%$} & {$68.12\%$}\\
{$10\%$} & {$80.36\%$} & {$74.09\%$} & {$81.39\%$} & {$70.50\%$} & {$79.65\%$} & {$68.08\%$}\\
{$20\%$} & {$80.12\%$} & {$74.14\%$} & {$80.71\%$} & {$69.96\%$} & {$79.59\%$} & {$68.10\%$}\\
{$30\%$} & {$79.89\%$} & {$73.50\%$} & {$79.28\%$} & {$68.75\%$} & {$79.37\%$} & {$68.09\%$}\\
{$40\%$} & {$78.43\%$} & {$73.57\%$} & {$77.13\%$} & {$68.60\%$} & {$78.96\%$} & {$67.91\%$}\\
{$50\%$} & {$70.29\%$} & {$59.58\%$} & {$73.46\%$} & {$63.96\%$} & {$76.97\%$} & {$66.64\%$}\\
{$60\%$} & {$59.58\%$} & {$52.84\%$} & {$71.12\%$} & {$63.42\%$} & {$72.91\%$} & {$62.03\%$}\\
{$70\%$} & {$50.64\%$} & {$50.26\%$} & {$67.22\%$} & {$60.79\%$} & {$62.64\%$} & {$47.87\%$}\\
{$80\%$} & {$47.93\%$} & {$51.92\%$} & {$60.99\%$} & {$59.24\%$} & {$47.54\%$} & {$29.71\%$}\\
{$90\%$} & {$47.90\%$} & {$51.88\%$} & {$55.86\%$} & {$59.59\%$} & {$35.17\%$} & {$21.59\%$}\\
\hline
\end{tabular}
\label{Table:6}
\end{table*}

\begin{table*}[!ht]
\small
 \centering
 \caption{Test accuracy and attack success rate difference after model pruning for graph classification task (COLLAB, W\_r)}
\begin{tabular}{c|c|c|c|c|c|c}
 \hline
\multirow{2}{*}{Pruning rate} & \multicolumn{2}{c|}{DiffPool} & \multicolumn{2}{c|}{GIN} & \multicolumn{2}{c}{GraphSAGE} \\
\cline{2-7}
 & {Test Acc.} & {Watermark Acc. Diff.} & {Test Acc.} & {Watermark Acc. Diff.} & {Test Acc.} & {Watermark Acc. Diff.}\\
\hline
{$0\%$} & {$80.71\%$} & {$69.45\%$} & {$81.63\%$} & {$63.67\%$} & {$79.88\%$} & {$68.41\%$}\\
{$10\%$} & {$80.69\%$} & {$69.51\%$} & {$81.66\%$} & {$63.09\%$} & {$79.89\%$} & {$69.01\%$}\\
{$20\%$} & {$80.55\%$} & {$69.38\%$} & {$81.49\%$} & {$60.03\%$} & {$79.90\%$} & {$68.92\%$}\\
{$30\%$} & {$80.15\%$} & {$69.41\%$} & {$81.44\%$} & {$62.57\%$} & {$79.69\%$} & {$68.21\%$}\\
{$40\%$} & {$79.28\%$} & {$69.03\%$} & {$80.84\%$} & {$61.47\%$} & {$79.57\%$} & {$68.32\%$}\\
{$50\%$} & {$76.36\%$} & {$55.56\%$} & {$79.24\%$} & {$38.20\%$} & {$79.34\%$} & {$68.30\%$}\\
{$60\%$} & {$64.80\%$} & {$34.73\%$} & {$76.55\%$} & {$12.73\%$} & {$77.91\%$} & {$68.25\%$}\\
{$70\%$} & {$47.63\%$} & {$6.94\%$} & {$70.30\%$} & {$12.73\%$} & {$72.64\%$} & {$68.14\%$}\\
{$80\%$} & {$36.60\%$} & {$6.94\%$} & {$63.52\%$} & {$12.73\%$} & {$57.77\%$} & {$54.73\%$}\\
{$90\%$} & {$32.53\%$} & {$0.00\%$} & {$42.34\%$} & {$0.00\%$} & {$37.26\%$} & {$34.21\%$}\\
\hline
\end{tabular}
\label{Table:6}
\end{table*}

\begin{table*}[!ht]
\small
 \centering
 \caption{Test accuracy and attack success rate difference after model pruning for graph classification task (REDDIT-BINARY, W\_t)}
\begin{tabular}{c|c|c|c|c|c|c}
 \hline
\multirow{2}{*}{Pruning rate} & \multicolumn{2}{c|}{DiffPool} & \multicolumn{2}{c|}{GIN} & \multicolumn{2}{c}{GraphSAGE} \\
\cline{2-7}
 & {Test Acc.} & {Watermark Acc. Diff.} & {Test Acc.} & {Watermark Acc. Diff.} & {Test Acc.} & {Watermark Acc. Diff.}\\
\hline
{$0\%$} & {$86.61\%$} & {$82.09\%$} & {$87.23\%$} & {$81.25\%$} & {$78.21\%$} & {$99.50\%$}\\
{$10\%$} & {$86.75\%$} & {$81.94\%$} & {$87.41\%$} & {$80.92\%$} & {$78.30\%$} & {$99.34\%$}\\
{$20\%$} & {$86.78\%$} & {$82.04\%$} & {$87.20\%$} & {$80.45\%$} & {$78.33\%$} & {$99.29\%$}\\
{$30\%$} & {$86.79\%$} & {$81.87\%$} & {$87.30\%$} & {$80.25\%$} & {$78.33\%$} & {$99.47\%$}\\
{$40\%$} & {$86.58\%$} & {$81.68\%$} & {$87.26\%$} & {$80.35\%$} & {$77.96\%$} & {$98.99\%$}\\
{$50\%$} & {$86.91\%$} & {$80.99\%$} & {$84.76\%$} & {$80.86\%$} & {$77.70\%$} & {$99.04\%$}\\
{$60\%$} & {$86.43\%$} & {$81.32\%$} & {$81.45\%$} & {$77.37\%$} & {$76.85\%$} & {$99.65\%$}\\
{$70\%$} & {$82.61\%$} & {$80.83\%$} & {$77.99\%$} & {$66.22\%$} & {$73.40\%$} & {$99.42\%$}\\
{$80\%$} & {$72.62\%$} & {$72.47\%$} & {$73.48\%$} & {$59.82\%$} & {$64.95\%$} & {$99.47\%$}\\
{$90\%$} & {$60.69\%$} & {$23.65\%$} & {$68.11\%$} & {$56.42\%$} & {$53.79\%$} & {$97.35\%$}\\
\hline
\end{tabular}
\label{Table:6}
\end{table*}

\begin{table*}[!ht]
\small
 \centering
 \caption{Test accuracy and attack success rate difference after model pruning for graph classification task (REDDIT-BINARY, W\_r)}
\begin{tabular}{c|c|c|c|c|c|c}
 \hline
\multirow{2}{*}{Pruning rate} & \multicolumn{2}{c|}{DiffPool} & \multicolumn{2}{c|}{GIN} & \multicolumn{2}{c}{GraphSAGE} \\
\cline{2-7}
 & {Test Acc.} & {Watermark Acc. Diff.} & {Test Acc.} & {Watermark Acc. Diff.} & {Test Acc.} & {Watermark Acc. Diff.}\\
\hline
{$0\%$} & {$86.55\%$} & {$55.72\%$} & {$87.08\%$} & {$53.21\%$} & {$77.95\%$} & {$51.25\%$}\\
{$10\%$} & {$86.55\%$} & {$55.53\%$} & {$87.05\%$} & {$53.26\%$} & {$77.94\%$} & {$50.91\%$}\\
{$20\%$} & {$86.58\%$} & {$55.12\%$} & {$87.11\%$} & {$53.01\%$} & {$77.89\%$} & {$51.13\%$}\\
{$30\%$} & {$86.24\%$} & {$55.53\%$} & {$86.84\%$} & {$52.86\%$} & {$77.77\%$} & {$51.04\%$}\\
{$40\%$} & {$86.42\%$} & {$55.54\%$} & {$85.92\%$} & {$52.95\%$} & {$77.74\%$} & {$50.86\%$}\\
{$50\%$} & {$86.55\%$} & {$55.76\%$} & {$84.98\%$} & {$52.94\%$} & {$77.48\%$} & {$50.12\%$}\\
{$60\%$} & {$85.70\%$} & {$54.86\%$} & {$83.57\%$} & {$50.26\%$} & {$77.56\%$} & {$50.95\%$}\\
{$70\%$} & {$82.89\%$} & {$50.15\%$} & {$80.72\%$} & {$30.90\%$} & {$76.34\%$} & {$51.24\%$}\\
{$80\%$} & {$74.39\%$} & {$44.95\%$} & {$76.22\%$} & {$36.89\%$} & {$72.43\%$} & {$50.85\%$}\\
{$90\%$} & {$63.94\%$} & {$23.89\%$} & {$70.56\%$} & {$31.39\%$} & {$59.67\%$} & {$51.12\%$}\\
\hline
\end{tabular}
\label{Table:6}
\end{table*}

\begin{table*}[!ht]
\small
 \centering
 \caption{Test accuracy and attack success rate difference after model pruning for node classification task (CiteSeer)}
\begin{tabular}{c|c|c|c|c|c|c}
 \hline
\multirow{2}{*}{Pruning rate} & \multicolumn{2}{c|}{GCN} & \multicolumn{2}{c|}{GAT} & \multicolumn{2}{c}{SAGE} \\
\cline{2-7}
 & {Test Acc.} & {Watermark Acc. Diff.} & {Test Acc.} & {Watermark Acc. Diff.} & {Test Acc.} & {Watermark Acc. Diff.}\\
\hline
{$0\%$} & {$74.48\%$} & {$99.78\%$} & {$78.57\%$} & {$99.16\%$} & {$80.20\%$} & {$93.14\%$}\\
{$10\%$} & {$74.50\%$} & {$99.75\%$} & {$78.55\%$} & {$99.13\%$} & {$80.25\%$} & {$93.17\%$}\\
{$20\%$} & {$74.42\%$} & {$99.72\%$} & {$78.57\%$} & {$99.09\%$} & {$80.34\%$} & {$93.09\%$}\\
{$30\%$} & {$74.47\%$} & {$99.70\%$} & {$78.42\%$} & {$99.11\%$} & {$80.24\%$} & {$93.13\%$}\\
{$40\%$} & {$74.45\%$} & {$99.65\%$} & {$78.57\%$} & {$99.14\%$} & {$80.28\%$} & {$93.17\%$}\\
{$50\%$} & {$74.41\%$} & {$99.61\%$} & {$78.49\%$} & {$99.06\%$} & {$80.45\%$} & {$93.07\%$}\\
{$60\%$} & {$74.35\%$} & {$99.54\%$} & {$78.35\%$} & {$99.13\%$} & {$75.32\%$} & {$82.06\%$}\\
{$70\%$} & {$74.22\%$} & {$99.31\%$} & {$78.32\%$} & {$99.07\%$} & {$74.27\%$} & {$48.79\%$}\\
{$80\%$} & {$73.93\%$} & {$99.04\%$} & {$78.08\%$} & {$98.97\%$} & {$73.20\%$} & {$15.29\%$}\\
{$90\%$} & {$72.93\%$} & {$98.25\%$} & {$77.59\%$} & {$98.41\%$} & {$72.00\%$} & {$7.73\%$}\\
\hline
\end{tabular}
\label{Table:6}
\end{table*}

\iffalse
\begin{table}[!ht]
\centering
\small
 \centering
 \caption{Accuracy difference on watermarked data for graph classification task ($r=0.15, \gamma=0.2, p=1.0$)}
\begin{subtable}[t]{0.48\textwidth}
\caption{\footnotesize NCI1}
\begin{tabular}{M{60pt}|M{40pt}|M{42pt}|M{40pt}}
 \hline
{Accuracy Difference} & {DiffPool} & {GIN} & {GraphSAGE} \\
 \hline
 \hline
 $D_{wm}^{t}$ & $88.11\%$ & $80.93\%$ & $91.28\%$ \\
 \hline
 $D_{wm}^{r}$ & $49.39\%$ & $44.25\%$ & $49.68\%$ \\
 \hline
\end{tabular}
\label{Table:asrd_graph_classification_a}
\end{subtable}

\begin{subtable}[t]{0.48\textwidth}
\caption{\footnotesize COLLAB}
\begin{tabular}{M{60pt}|M{40pt}|M{42pt}|M{40pt}}
 \hline
{Accuracy Difference} & {DiffPool} & {GIN} & {GraphSAGE} \\
 \hline
 \hline
 $D_{wm}^{t}$ & $74.16\%$ & $70.47\%$ & $68.12\%$ \\
 \hline
 $D_{wm}^{r}$ & $69.45\%$ & $63.67\%$ & $68.41\%$ \\
 \hline
\end{tabular}
\label{Table:asrd_graph_classification_b}
\end{subtable}

\begin{subtable}[t]{0.48\textwidth}
\caption{\footnotesize REDDIT-BINARY}
\begin{tabular}{M{60pt}|M{40pt}|M{42pt}|M{40pt}}
 \hline
{Accuracy Difference} & {DiffPool} & {GIN} & {GraphSAGE} \\
 \hline
 \hline
 $D_{wm}^{t}$ & $82.09\%$ & $81.25\%$ & $99.50\%$ \\
 \hline
 $D_{wm}^{r}$ & $55.72\%$ & $53.21\%$ & $51.25\%$ \\
 \hline
\end{tabular}
\label{Table:asrd_graph_classification_c}
\end{subtable}
\label{Table:asrd_graph_classification}
\end{table}
\fi

\iffalse
\begin{table}[!ht]
\small
 \centering
 \caption{Test accuracy for node classification task}
\begin{subtable}{0.5\textwidth}
\caption{\footnotesize Cora}
\centering
\begin{tabular}{c|c|c|c}
 \hline
{Test Accuracy} & {GCN} & {GAT} & {SAGE}\\
 \hline
 \hline
 {Clean Model} & $87.21\%$ & $87.94\%$ & $84.04\%$\\
 \hline
 $D_{wm}^{t}$ & $86.82\%$ & $86.98\%$ & $83.88\%$\\
 \hline
\end{tabular}
\label{Table:test_acc_node_classification_a}
\end{subtable}

\begin{subtable}[t]{0.5\textwidth}
\centering
\caption{\footnotesize CiteSeer}
\begin{tabular}{c|c|c|c}
 \hline
{Test Accuracy} & {GCN} & {GAT} &{SAGE} \\
 \hline
 \hline
 {Clean Model} & $78.67\%$ & $80.33\%$ & $75.12\%$\\
 \hline
 $D_{wm}^{t}$ & $78.23\%$ & $79.57\%$ & $75.04\%$\\
 \hline
\end{tabular}
\label{Table:test_acc_node_classification_b}
\end{subtable}
\label{Table:test_acc_node_classification}
\end{table}
\fi

\iffalse
\begin{table}[!ht]
\small
 \centering
 \caption{Accuracy difference on watermarked data after fine-tuning for the graph classification task}
\begin{subtable}[t]{0.48\textwidth}
\caption{\footnotesize NCI1}
\begin{tabular}{M{50pt}|M{40pt}|M{42pt}|M{40pt}}
 \hline
{Accuracy Difference} & {DiffPool} & {GIN} & {GraphSAGE} \\
 \hline
 \hline
 $D_{wm}^{t}$ & $86.42\%$ & $79.31\%$ & $90.10\%$ \\
 \hline
 $D_{wm}^{r}$ & $47.64\%$ & $43.28\%$ & $49.09\%$ \\
 \hline
\end{tabular}
\label{Table:asrd_fine_tuning_graph_classification_a}
\end{subtable}


\begin{subtable}[t]{0.48\textwidth}
\caption{\footnotesize COLLAB}
\begin{tabular}{M{50pt}|M{40pt}|M{42pt}|M{40pt}}
 \hline
{Accuracy Difference} & {DiffPool} & {GIN} & {GraphSAGE} \\
 \hline
 \hline
 $D_{wm}^{t}$ & $72.50\%$ & $68.22\%$ & $65.67\%$ \\
 \hline
 $D_{wm}^{r}$ & $68.00\%$ & $60.84\%$ & $65.93\%$ \\
 \hline
\end{tabular}
\label{Table:asrd_fine_tuning_graph_classification_b}
\end{subtable}

\begin{subtable}[t]{0.48\textwidth}
\caption{\footnotesize REDDIT-BINARY}
\begin{tabular}{M{50pt}|M{40pt}|M{42pt}|M{40pt}}
 \hline
{Accuracy Difference} & {DiffPool} & {GIN} & {GraphSAGE} \\
 \hline
 \hline
 $D_{wm}^{t}$ & $79.50\%$ & $79.22\%$ & $97.67\%$ \\
 \hline
 $D_{wm}^{r}$ & $53.91\%$ & $52.04\%$ & $49.94\%$ \\
 \hline
\end{tabular}
\label{Table:asrd_fine_tuning_graph_classification_b}
\end{subtable}
\label{Table:asrd_fine_tuning_graph_classification}
\end{table}
\fi

\iffalse
\begin{table}[!ht]
\centering
\small
 \centering
 \caption{Test accuracy after fine-tuning for graph classification task ($r=0.15, \gamma=0.2, p=1.0$). }
\begin{subtable}[t]{0.48\textwidth}
\caption{\footnotesize NCI1}
\begin{tabular}{M{50pt}|M{40pt}|M{40pt}|M{40pt}}
 \hline
{Test Accuracy} & {DiffPool} & {GIN} & {GraphSAGE} \\
 \hline
 \hline
 $D_{wm}^{t}$ & $73.61\%$ & $75.05\%$ & $71.92\%$\\
 \hline
 $D_{wm}^{r}$ & $77.15\%$ & $77.84\%$ & $74.89\%$\\
 
 \hline
\end{tabular}
\label{Table:test_acc_fine_tuning_graph_classification_a}
\end{subtable}


\begin{subtable}[t]{0.48\textwidth}
\caption{\footnotesize COLLAB}
\begin{tabular}{M{50pt}|M{40pt}|M{40pt}|M{40pt}}
 \hline
{Test Accuracy} & {DiffPool} & {GIN} & {GraphSAGE} \\
 \hline
 \hline
 $D_{wm}^{t}$ & $76.10\%$ & $77.63\%$ & $75.93\%$\\
 \cline{1-4}
 $D_{wm}^{r}$ & $80.67\%$ & $80.92\%$ & $78.31\%$\\
 \hline
\end{tabular}
\label{Table:test_acc_fine_tuning_graph_classification_b}
\end{subtable}

\begin{subtable}[t]{0.48\textwidth}
\caption{\footnotesize REDDIT-BINARY}
\begin{tabular}{M{50pt}|M{40pt}|M{40pt}|M{40pt}}
 \hline
{Test Accuracy} & {DiffPool} & {GIN} & {GraphSAGE} \\
 \hline
 \hline
 $D_{wm}^{t}$ & $82.10\%$ & $80.63\%$ & $73.82\%$\\
 \cline{1-4}
 $D_{wm}^{r}$ & $86.20\%$ & $86.89\%$ & $77.85\%$\\
 \hline
\end{tabular}
\label{Table:test_acc_fine_tuning_graph_classification_c}
\end{subtable}
\label{Table:test_acc_fine_tuning_graph_classification}
\end{table}
\fi

\iffalse
\begin{table*}[!ht]
\small
 \centering
 \caption{Watermarking performance on graph classification task after model pruning (NCI1, $D_{wm}^{t}$)}
\begin{tabular}{c|c|c|c|c|c|c}
 \hline
\multirow{2}{*}{Pruning rate} & \multicolumn{2}{c|}{DiffPool} & \multicolumn{2}{c|}{GIN} & \multicolumn{2}{c}{GraphSAGE} \\
\cline{2-7}
 & {Test Acc.} & {Watermark Acc. Diff.} & {Test Acc.} & {Watermark Acc. Diff.} & {Test Acc.} & {Watermark Acc. Diff.}\\
\hline
{$0\%$} & {$77.80\%$} & {$88.11\%$} & {$78.18\%$} & {$80.93\%$} & {$75.01\%$} & {$91.28\%$}\\
{$10\%$} & {$77.77\%$} & {$87.94\%$} & {$78.21\%$} & {$80.56\%$} & {$74.66\%$} & {$91.24\%$}\\
{$20\%$} & {$77.72\%$} & {$87.89\%$} & {$77.79\%$} & {$80.42\%$} & {$74.77\%$} & {$91.01\%$}\\
{$30\%$} & {$77.61\%$} & {$87.12\%$} & {$77.24\%$} & {$80.01\%$} & {$73.56\%$} & {$90.96\%$}\\
{$40\%$} & {$76.79\%$} & {$83.85\%$} & {$72.93\%$} & {$79.93\%$} & {$73.32\%$} & {$90.89\%$}\\
{$50\%$} & {$70.77\%$} & {$79.31\%$} & {$63.34\%$} & {$74.56\%$} & {$70.08\%$} & {$90.76\%$}\\
{$60\%$} & {$60.17\%$} & {$61.34\%$} & {$57.60\%$} & {$67.13\%$} & {$61.62\%$} & {$90.83\%$}\\
{$70\%$} & {$52.46\%$} & {$26.73\%$} & {$56.39\%$} & {$64.50\%$} & {$53.58\%$} & {$90.56\%$}\\
{$80\%$} & {$50.66\%$} & {$0.00\%$} & {$54.11\%$} & {$53.31 \%$} & {$50.26\%$} & {$87.35\%$}\\
{$90\%$} & {$50.66\%$} & {$0.00\%$} & {$52.00\%$} & {$49.37 \%$} & {$49.67\%$} & {$75.08\%$}\\
\hline
\end{tabular}
\label{Table:6}
\end{table*}

\begin{table*}[!ht]
\small
 \centering
 \caption{Watermarking performance on graph classification task after model pruning (NCI1, $D_{wm}^{r}$)}
\begin{tabular}{c|c|c|c|c|c|c}
 \hline
\multirow{2}{*}{Pruning rate} & \multicolumn{2}{c|}{DiffPool} & \multicolumn{2}{c|}{GIN} & \multicolumn{2}{c}{GraphSAGE} \\
\cline{2-7}
 & {Test Acc.} & {Watermark Acc. Diff.} & {Test Acc.} & {Watermark Acc. Diff.} & {Test Acc.} & {Watermark Acc. Diff.}\\
\hline
{$0\%$} & {$77.85\%$} & {$49.39\%$} & {$77.80\%$} & {$44.25\%$} & {$74.79\%$} & {$49.68\%$}\\
{$10\%$} & {$77.86\%$} & {$49.35\%$} & {$77.81\%$} & {$44.02\%$} & {$74.83\%$} & {$49.57\%$}\\
{$20\%$} & {$77.84\%$} & {$49.21\%$} & {$77.62\%$} & {$44.15\%$} & {$74.46\%$} & {$49.60\%$}\\
{$30\%$} & {$77.69\%$} & {$49.43\%$} & {$76.95\%$} & {$44.27\%$} & {$73.93\%$} & {$49.47\%$}\\
{$40\%$} & {$77.25\%$} & {$49.31\%$} & {$71.76\%$} & {$44.14\%$} & {$72.36\%$} & {$49.39\%$}\\
{$50\%$} & {$74.71\%$} & {$49.16\%$} & {$61.31\%$} & {$43.87\%$} & {$70.12\%$} & {$49.46\%$}\\
{$60\%$} & {$66.46\%$} & {$38.56\%$} & {$56.66\%$} & {$42.07\%$} & {$62.71\%$} & {$49.37\%$}\\
{$70\%$} & {$55.14\%$} & {$29.66\%$} & {$52.79\%$} & {$43.09\%$} & {$52.91\%$} & {$49.40\%$}\\
{$80\%$} & {$51.35\%$} & {$14.66\%$} & {$51.55\%$} & {$42.29\%$} & {$51.10\%$} & {$49.37\%$}\\
{$90\%$} & {$50.36\%$} & {$4.95\%$} & {$50.47\%$} & {$43.18\%$} & {$49.07\%$} & {$34.66\%$}\\
\hline
\end{tabular}
\label{Table:6}
\end{table*}
\fi

% knowledge distillation
 NCI1 & $85.41 | 47.83$ & $78.50 | 42.92$ & $88.54 | 48.19$ \\
 \hline
 COLLAB & $71.90 | 67.37$ & $67.92 | 61.76$ & $65.96 | 66.36$ \\
 \hline 
 REDDIT-BINARY & $79.63 | 54.05$ & $78.82 | 51.62$ & $96.52 | 49.71$ \\
 \hline
 
 Cora & $96.83 | 88.22$ & $92.35 | 86.28$ & $96.94 | 82.19$\\
 \hline
 CiteSeer & $98.81 | 78.26$ & $99.13 | 73.65$ & $99.57 | 73.54$\\
 \hline 
 
 % fine-tuning
  NCI1 & $86.42 | 47.64$ & $79.31 | 43.28$ & $90.10 | 49.09$ \\
 \hline
 COLLAB & $72.50 | 68.00$ & $68.22 | 60.84$ & $65.67 | 65.93$ \\
 \hline 
 REDDIT-BINARY & $79.50 | 53.91$ & $79.22 | 52.04$ & $97.67 | 49.94$ \\
 \hline
 
 Cora & $96.22$ & $83.56$  \\
 \hline
 CiteSeer & $99.72$ & $75.10$ \\
 \hline
 
 % model pruning
 % NCI1
 %{$0\% $} & {$ 77.80\% $ | $ 77.85\% $} & {$ 88.11\% $ | $ 49.39\% $} & {$ 78.18\% $ | $ 77.80\% $} & {$ 80.93\% $ | $ 44.25\% $} & {$ 75.01\% $ | $ 74.79\% $} & {$ 91.28\% $ | $ 49.68\%$} \\
{$10\%$} & {$77.77\%|77.86\%$} & {$87.94\%|49.35\%$} & {$78.21\%|77.81\%$} & {$80.56\%|44.02\%$} & {$74.66\%|74.83\%$} & {$91.24\%|49.57\%$} \\
{$20\%$} & {$77.72\%|77.84\%$} & {$87.89\%|49.21\%$} & {$77.79\%|77.62\%$} & {$80.42\%|44.15\%$} & {$74.77\%|74.46\%$} & {$91.01\%|49.60\%$} \\
{$30\%$} & {$77.61\%|77.69\%$} & {$87.12\%|49.43\%$} & {$77.24\%|76.95\%$} & {$80.01\%|44.27\%$} & {$73.56\%|73.93\%$} & {$90.96\%|49.47\%$} \\
{$40\%$} & {$76.79\%|77.25\%$} & {$87.10\%|49.31\%$} & {$72.93\%|71.76\%$} & {$79.93\%|44.14\%$} & {$73.32\%|72.36\%$} & {$90.89\%|49.39\%$} \\
{$50\%$} & {$70.77\%|74.71\%$} & {$79.31\%|49.16\%$} & {$63.34\%|61.31\%$} & {$74.56\%|43.87\%$} & {$70.08\%|70.12\%$} & {$90.76\%|49.46\%$} \\
{$60\%$} & {$60.17\%|66.46\%$} & {$61.34\%|38.56\%$} & {$57.60\%|56.66\%$} & {$67.13\%|42.07\%$} & {$61.62\%|62.71\%$} & {$90.83\%|49.37\%$} \\
{$70\%$} & {$52.46\%|55.14\%$} & {$26.73\%|29.66\%$} & {$56.39\%|52.79\%$} & {$64.50\%|43.09\%$} & {$53.58\%|52.91\%$} & {$90.56\%|49.40\%$} \\
{$80\%$} & {$50.66\%|51.35\%$} & {$0.00\%|14.66\%$} & {$54.11\%|51.55\%$} & {$53.31\%|42.29\%$} & {$50.26\%|51.10\%$} & {$87.35\%|49.37\%$} \\
{$90\%$} & {$50.66\%|50.36\%$} & {$0.00\%|4.95\%$} & {$52.00\%|50.47\%$} & {$49.37\%|43.18\%$} & {$49.67\%|49.07\%$} & {$75.08\%|34.66\%$} \\
\hline

% COLLAB
{$10\%$} & {$80.36\%|80.69\%$} & {$74.09\%|69.51\%$} & {$81.39\%|81.66\%$} & {$70.50\%|63.09\%$} & {$79.65\%|79.89\%$} & {$68.08\%|69.01\%$} \\
{$20\%$} & {$80.12\%|80.55\%$} & {$74.14\%|69.38\%$} & {$80.71\%|81.49\%$} & {$69.96\%|63.03\%$} & {$79.59\%|79.90\%$} & {$68.10\%|68.92\%$} \\
{$30\%$} & {$79.89\%|80.15\%$} & {$73.50\%|69.41\%$} & {$79.28\%|81.44\%$} & {$68.75\%|62.57\%$} & {$79.37\%|79.69\%$} & {$68.09\%|68.21\%$} \\
{$40\%$} & {$78.43\%|79.28\%$} & {$73.57\%|69.03\%$} & {$77.13\%|80.84\%$} & {$68.60\%|61.47\%$} & {$78.96\%|79.57\%$} & {$67.91\%|68.32\%$} \\
{$50\%$} & {$70.29\%|76.36\%$} & {$59.58\%|55.56\%$} & {$73.46\%|79.24\%$} & {$63.96\%|38.20\%$} & {$76.97\%|79.34\%$} & {$66.64\%|68.30\%$} \\
{$60\%$} & {$59.58\%|64.80\%$} & {$52.84\%|34.73\%$} & {$71.12\%|76.55\%$} & {$63.42\%|12.73\%$} & {$72.91\%|77.91\%$} & {$62.03\%|68.25\%$} \\
{$70\%$} & {$50.64\%|47.63\%$} & {$50.26\%|6.94\%$} & {$67.22\%|70.30\%$} & {$60.79\%|12.73\%$} & {$62.64\%|72.64\%$} & {$47.87\%|68.14\%$} \\
{$80\%$} & {$47.93\%|36.60\%$} & {$51.92\%|6.94\%$} & {$60.99\%|63.52\%$} & {$59.24\%|12.73\%$} & {$47.54\%|57.77\%$} & {$29.71\%|54.73\%$} \\
{$90\%$} & {$47.90\%|32.53\%$} & {$51.88\%|0.00\%$} & {$55.86\%|42.34\%$} & {$59.59\%|0.00\%$} & {$35.17\%|37.26\%$} & {$21.59\%|34.21\%$} \\

% REDDIT-BINARY
{$10\%$} & {$86.75\%|86.55\%$} & {$81.94\%|55.53\%$} & {$87.41\%|87.05\%$} & {$80.92\%|53.26\%$} & {$78.30\%|77.94\%$} & {$99.34\%|50.91\%$} \\
{$20\%$} & {$86.78\%|86.58\%$} & {$82.04\%|55.12\%$} & {$87.20\%|87.11\%$} & {$80.45\%|53.01\%$} & {$78.33\%|77.89\%$} & {$99.29\%|51.13\%$} \\
{$30\%$} & {$86.79\%|86.24\%$} & {$81.87\%|55.53\%$} & {$87.30\%|86.84\%$} & {$80.25\%|52.86\%$} & {$78.33\%|77.77\%$} & {$99.47\%|51.04\%$} \\
{$40\%$} & {$86.58\%|86.42\%$} & {$81.68\%|55.54\%$} & {$87.26\%|85.92\%$} & {$80.35\%|52.95\%$} & {$77.96\%|77.74\%$} & {$98.99\%|50.86\%$} \\
{$50\%$} & {$86.91\%|86.55\%$} & {$80.99\%|55.76\%$} & {$84.76\%|84.98\%$} & {$80.86\%|52.94\%$} & {$77.70\%|77.48\%$} & {$99.04\%|50.12\%$} \\
{$60\%$} & {$86.43\%|85.70\%$} & {$81.32\%|54.86\%$} & {$81.45\%|83.57\%$} & {$77.37\%|50.26\%$} & {$76.85\%|77.56\%$} & {$99.65\%|50.95\%$} \\
{$70\%$} & {$82.61\%|82.89\%$} & {$80.83\%|50.15\%$} & {$77.99\%|80.72\%$} & {$66.22\%|30.90\%$} & {$73.40\%|76.34\%$} & {$99.42\%|51.24\%$} \\
{$80\%$} & {$72.62\%|74.39\%$} & {$72.47\%|44.95\%$} & {$73.48\%|76.22\%$} & {$59.82\%|36.89\%$} & {$64.95\%|72.43\%$} & {$99.47\%|50.85\%$} \\
{$90\%$} & {$60.69\%|63.94\%$} & {$23.65\%|23.89\%$} & {$68.11\%|70.56\%$} & {$56.42\%|31.39\%$} & {$53.79\%|59.67\%$} & {$97.35\%|51.12\%$} \\

% Cora
{$10\%$} & {$86.51\%$} & {$96.70\%$} & {$85.23\%$} & {$90.42\%$} & {$83.40\%$} & {$97.33\%$}\\
{$20\%$} & {$86.49\%$} & {$95.69\%$} & {$85.22\%$} & {$90.17\%$} & {$83.37\%$} & {$97.29\%$}\\
{$30\%$} & {$86.24\%$} & {$95.46\%$} & {$85.26\%$} & {$89.83\%$} & {$83.24\%$} & {$96.94\%$}\\
{$40\%$} & {$85.68\%$} & {$95.39\%$} & {$85.24\%$} & {$89.17\%$} & {$82.45\%$} & {$95.83\%$}\\
{$50\%$} & {$83.63\%$} & {$94.58\%$} & {$85.29\%$} & {$88.92\%$} & {$82.35\%$} & {$95.79\%$}\\
{$60\%$} & {$82.60\%$} & {$94.33\%$} & {$85.28\%$} & {$88.17\%$} & {$80.94\%$} & {$95.75\%$}\\
{$70\%$} & {$82.52\%$} & {$93.89\%$} & {$85.25\%$} & {$87.06\%$} & {$80.37\%$} & {$69.19\%$}\\
{$80\%$} & {$82.41\%$} & {$93.59\%$} & {$85.19\%$} & {$86.83\%$} & {$78.20\%$} & {$40.19\%$}\\
{$90\%$} & {$82.20\%$} & {$87.83\%$} & {$84.97\%$} & {$86.67\%$} & {$72.00\%$} & {$32.35\%$}\\

% CiteSeer
{$10\%$} & {$74.50\%$} & {$99.75\%$} & {$78.55\%$} & {$99.13\%$} & {$80.25\%$} & {$93.17\%$}\\
{$20\%$} & {$74.42\%$} & {$99.72\%$} & {$78.42\%$} & {$99.09\%$} & {$80.34\%$} & {$93.09\%$}\\
{$30\%$} & {$74.47\%$} & {$99.70\%$} & {$78.57\%$} & {$99.11\%$} & {$80.24\%$} & {$93.13\%$}\\
{$40\%$} & {$74.45\%$} & {$99.65\%$} & {$78.49\%$} & {$99.14\%$} & {$80.28\%$} & {$93.17\%$}\\
{$50\%$} & {$74.41\%$} & {$99.61\%$} & {$78.51\%$} & {$99.06\%$} & {$80.45\%$} & {$93.07\%$}\\
{$60\%$} & {$74.35\%$} & {$99.54\%$} & {$78.35\%$} & {$99.13\%$} & {$75.32\%$} & {$82.06\%$}\\
{$70\%$} & {$74.22\%$} & {$99.31\%$} & {$78.32\%$} & {$99.07\%$} & {$74.27\%$} & {$48.79\%$}\\
{$80\%$} & {$73.93\%$} & {$99.04\%$} & {$78.08\%$} & {$98.97\%$} & {$73.20\%$} & {$15.29\%$}\\
{$90\%$} & {$72.93\%$} & {$98.25\%$} & {$77.59\%$} & {$98.41\%$} & {$72.00\%$} & {$7.73\%$}\\

% fine-pruning
% NCI1
{$10\%$} & {$81.32\% | 77.20\%$} & {$88.11\% | 49.39\%$} & {$82.32\% | 79.18\%$} & {$80.84\% | 44.25\%$} & {$74.96\% | 75.71\%$} & {$91.64\% | 49.84\%$}\\
{$20\%$} & {$81.00\% | 77.43\%$} & {$86.88\% | 46.05\%$} & {$82.01\% | 79.12\%$} & {$80.79\% | 43.09\%$} & {$75.00\% | 75.51\%$} & {$91.57\% | 49.21\%$}\\
{$30\%$} & {$81.16\% | 77.52\%$} & {$85.88\% | 42.59\%$} & {$81.57\% | 78.99\%$} & {$80.67\% | 43.10\%$} & {$74.58\% | 75.50\%$} & {$90.97\% | 49.54\%$}\\
{$40\%$} & {$80.35\% | 77.43\%$} & {$85.80\% | 42.39\%$} & {$81.12\% | 79.06\%$} & {$80.65\% | 43.18\%$} & {$73.74\% | 75.43\%$} & {$91.08\% | 48.94\%$}\\
{$50\%$} & {$79.20\% | 77.58\%$} & {$82.20\% | 41.56\%$} & {$80.10\% | 78.98\%$} & {$80.74\% | 42.96\%$} & {$72.37\% | 75.66\%$} & {$90.89\% | 48.72\%$}\\
{$60\%$} & {$76.83\% | 77.48\%$} & {$80.78\% | 40.75\%$} & {$78.93\% | 78.92\%$} & {$80.63\% | 42.81\%$} & {$68.01\% | 75.17\%$} & {$91.28\% | 48.67\%$}\\
{$70\%$} & {$75.14\% | 77.48\%$} & {$80.52\% | 37.25\%$} & {$75.74\% | 78.70\%$} & {$80.49\% | 42.74\%$} & {$61.86\% | 74.25\%$} & {$90.84\% | 48.74\%$}\\
{$80\%$} & {$69.73\% | 77.20\%$} & {$74.09\% | 36.82\%$} & {$72.01\% | 77.78\%$} & {$80.53\% | 42.94\%$} & {$55.62\% | 73.95\%$} & {$91.23\% | 48.69\%$}\\
{$90\%$} & {$66.71\% | 75.21\%$} & {$59.84\% | 36.40\%$} & {$66.93\% | 75.89\%$} & {$73.24\% | 36.70\%$} & {$50.71\% | 66.37\%$} & {$91.09\% | 25.47\%$}\\

%COLLAB
{$10\%$} & {$71.77\% | 92.62\%$} & {$74.16\% | 69.45\%$} & {$69.55\% | 87.42\%$} & {$70.47\% | 63.67\%$} & {$69.07\% | 92.06\%$} & {$68.12\% | 68.41\%$}\\
{$20\%$} & {$72.07\% | 92.71\%$} & {$74.16\% | 52.09\%$} & {$69.52\% | 87.56\%$} & {$70.29\% | 57.30\%$} & {$69.39\% | 91.98\%$} & {$68.12\% | 67.01\%$}\\
{$30\%$} & {$70.50\% | 93.07\%$} & {$74.12\% | 43.41\%$} & {$68.04\% | 87.48\%$} & {$69.23\% | 56.97\%$} & {$69.20\% | 92.00\%$} & {$68.10\% | 57.01\%$}\\
{$40\%$} & {$65.29\% | 93.08\%$} & {$74.12\% | 43.38\%$} & {$65.80\% | 87.07\%$} & {$66.50\% | 56.78\%$} & {$69.38\% | 91.93\%$} & {$68.10\% | 58.94\%$}\\
{$50\%$} & {$60.62\% | 93.28\%$} & {$74.10\% | 43.24\%$} & {$62.80\% | 86.84\%$} & {$66.34\% | 25.47\%$} & {$69.20\% | 91.84\%$} & {$68.09\% | 57.84\%$}\\
{$60\%$} & {$56.44\% | 93.25\%$} & {$74.01\% | 43.16\%$} & {$57.29\% | 86.10\%$} & {$65.71\% | 19.10\%$} & {$65.23\% | 91.87\%$} & {$67.34\% | 57.59\%$}\\
{$70\%$} & {$53.53\% | 93.35\%$} & {$73.52\% | 34.72\%$} & {$53.28\% | 86.47\%$} & {$65.12\% | 18.54\%$} & {$60.01\% | 91.59\%$} & {$67.19\% | 56.84\%$}\\
{$80\%$} & {$52.39\% | 93.16\%$} & {$73.25\% | 34.64\%$} & {$52.93\% | 85.95\%$} & {$63.83\% | 12.73\%$} & {$54.77\% | 91.00\%$} & {$66.60\% | 55.74\%$}\\
{$90\%$} & {$52.45\% | 92.70\%$} & {$72.99\% | 34.59\%$} & {$52.44\% | 84.64\%$} & {$63.30\% | 12.39\%$} & {$51.94\% | 89.87\%$} & {$65.42\% | 45.61\%$}\\

%REDDIT-BINARY
{$10\%$} & {$83.29\% | 95.52\%$} & {$82.09\% | 55.72\%$} & {$84.83\% | 93.35\%$} & {$81.25\% | 53.21\%$} & {$73.76\% | 88.37\%$} & {$99.50\% | 51.25\%$}\\
{$20\%$} & {$83.02\% | 95.52\%$} & {$79.91\% | 53.26\%$} & {$84.47\% | 93.03\%$} & {$79.84\% | 50.48\%$} & {$73.67\% | 87.86\%$} & {$98.95\% | 50.94\%$}\\
{$30\%$} & {$83.20\% | 95.52\%$} & {$79.43\% | 53.21\%$} & {$85.97\% | 92.82\%$} & {$75.89\% | 52.52\%$} & {$73.85\% | 87.77\%$} & {$99.27\% | 51.36\%$}\\
{$40\%$} & {$84.84\% | 95.67\%$} & {$78.34\% | 52.78\%$} & {$85.10\% | 93.06\%$} & {$75.78\% | 51.79\%$} & {$73.94\% | 87.83\%$} & {$98.79\% | 51.24\%$}\\
{$50\%$} & {$84.45\% | 95.91\%$} & {$78.00\% | 52.73\%$} & {$84.65\% | 93.09\%$} & {$76.24\% | 51.36\%$} & {$73.88\% | 88.07\%$} & {$98.67\% | 50.58\%$}\\
{$60\%$} & {$84.72\% | 96.15\%$} & {$66.61\% | 51.87\%$} & {$83.51\% | 93.20\%$} & {$55.87\% | 36.57\%$} & {$73.49\% | 87.86\%$} & {$98.45\% | 50.84\%$}\\
{$70\%$} & {$83.62\% | 95.94\%$} & {$65.93\% | 50.71\%$} & {$83.00\% | 93.65\%$} & {$54.58\% | 36.24\%$} & {$72.60\% | 87.56\%$} & {$98.39\% | 50.46\%$}\\
{$80\%$} & {$82.66\% | 95.73\%$} & {$63.41\% | 49.89\%$} & {$80.18\% | 93.71\%$} & {$24.45\% | 35.35\%$} & {$72.30\% | 88.58\%$} & {$98.49\% | 50.37\%$}\\
{$90\%$} & {$78.17\% | 95.94\%$} & {$46.57\% | 41.76\%$} & {$73.74\% | 93.74\%$} & {$17.98\% | 33.69\%$} & {$69.07\% | 90.00\%$} & {$98.51\% | 50.43\%$}\\

%Cora & CiteSeer
{$10\%$} & {$84.04\%$} & {$97.41\%$} & {$72.12\%$} & {$99.54\%$}\\
{$20\%$} & {$83.45\%$} & {$97.54\%$} & {$71.37\%$} & {$99.76\%$}\\
{$30\%$} & {$83.06\%$} & {$97.24\%$} & {$71.00\%$} & {$99.41\%$}\\
{$40\%$} & {$83.45\%$} & {$96.94\%$} & {$71.56\%$} & {$99.86\%$}\\
{$50\%$} & {$83.26\%$} & {$96.78\%$} & {$71.93\%$} & {$99.92\%$}\\
{$60\%$} & {$82.48\%$} & {$95.77\%$} & {$71.56\%$} & {$88.23\%$}\\
{$70\%$} & {$83.06\%$} & {$66.89\%$} & {$71.19\%$} & {$50.87\%$}\\
{$80\%$} & {$71.70\%$} & {$33.95\%$} & {$61.93\%$} & {$16.02\%$}\\
{$90\%$} & {$64.87\%$} & {$24.42\%$} & {$56.55\%$} & {$8.13\%$}\\

\begin{theorem}
\label{theorem:watermark_acc_diff_threshould}
Given a suspicious model $m^{'}$ and a clean model $m_c$, with the number of queries to $m^{'}$ and $m_c$ at $q$, if the watermark accuracy difference $\delta$ satisfies the following formula:
\[ \sqrt{q-1}\cdot \delta - \sqrt{(\delta+\beta)-(\delta+\beta)^2}\cdot t_{\tau } > 0,\]
the model owner can reject the null hypothesis $\mathcal{H}_0$ at the significance level $1-\tau$, where $\beta$ is the watermark accuracy of the clean model and $t_\tau$ is the $\tau$ quantile of the t distribution with $q-1$ degrees of freedom.
\end{theorem}
